Active Evaluation: Efficient NLG Evaluation with Few Pairwise Comparisons

Recent studies have shown the advantages of evaluating NLG systems using pairwise comparisons as opposed to direct assessment. Given $k$ systems, a naive approach for identifying the top-ranked system would be to uniformly obtain pairwise comparisons from all ${k \choose 2}$ pairs of systems. However, this can be very expensive as the number of human annotations required would grow quadratically with $k$. In this work, we introduce Active Evaluation, a framework to efficiently identify the top-ranked system by actively choosing system pairs for comparison using dueling bandit algorithms. We perform extensive experiments with 13 dueling bandits algorithms on 13 NLG evaluation datasets spanning 5 tasks and show that the number of human annotations can be reduced by 80%. To further reduce the number of human annotations, we propose model-based dueling bandit algorithms which combine automatic evaluation metrics with human evaluations. Specifically, we eliminate sub-optimal systems even before the human annotation process and perform human evaluations only on test examples where the automatic metric is highly uncertain. This reduces the number of human annotations required further by 89%. In effect, we show that identifying the top-ranked system requires only a few hundred human annotations, which grow linearly with $k$. Lastly, we provide practical recommendations and best practices to identify the top-ranked system efficiently. Our code has been made publicly available at https://github.com/akashkm99/duelnlg

==> discussion.tex <==
\section{Discussion}
We further analyze the factors affecting the query complexity of dueling bandit algorithms \textit{viz.} number of NLG systems, automatic evaluation metrics, and hyperparameters of model-based algorithms. Lastly, we discuss the robustness of dueling bandit algorithms to delays in feedback arising when multiple human annotators are used in parallel. 
\label{sec:discussion}
\subsection{Effect of number of NLG systems}
We analyze the variations in query complexity with the number of NLG systems on the ParaBank dataset, originally with 28 NLG systems. We choose a subset of $k$ NLG systems and compute the query complexity in finding the top rank system among these $k$ systems. As shown in figure \ref{fig:number_of_nlg_systems}, the query complexity of the model-free uniform exploration algorithm grows quadratically since it explores all system pairs equally. However, for (model-free) dueling bandit algorithms that use efficient exploration strategies such as RCS, RUCB, and RMED, we observe that query complexity is much lower and only varies as $O(k)$. We observed similar trends with model-based algorithms but don't report them here due to space constraints.
% \MK{Are we talking about model free or model based here? If its model free then should we have a similar plot for model based also?}.
\subsection{Comparison between Evaluation Metrics}
We examine the effect of using different evaluation metrics in our random mixing algorithm with RMED in figure \ref{fig:comparison_metrics}. We notice that using the Bleu metric, which only achieves an accuracy of 41.5\% in MT, leads to an increase in query complexity in many MT datasets because of its inaccurate preference feedback. We observe similar trends for Embedding Average in a few datasets, but on average, we notice a decrease in query complexity by 7.95\% relative to the model-free RMED algorithm. With Laser, MoverScore, and BertScore, we obtain an average reduction in query complexity by 51.27\%, 57.34\%, and 50.85\%, respectively, relative to model-free RMED. The improvements are even greater with Bleurt and Electra at 70.43\% and 73.15\%, respectively.
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/wmt-bleurt-rand-mix-bald.png}
%     \caption{Variation in query complexity with Mixing probability in Random Mixing with Bleurt on the left and with BALD threshold in Uncertainty-aware Selection (BALD) with Bleurt on the right}
%     \label{fig:hyperparameter_variation}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/wmt15-deu-eng-rand-mix.png}
%     \caption{Prediction accuracy vs number of human annotations collected for random mixing with Bluert and Bleu for different mixing probability $\gamma_{mix}$ on the WMT 15 deu-eng dataset}
%     \label{fig:bleurt_vs_bleu}
% \end{figure}
% \subsection{Effect of Hyperparameters}
% We study how hyperparameters in our proposed model-based algorithms affect the query complexity. In figure \ref{fig:hyperparameter_variation}, we show the effect of mixing probability $\gamma_{mix}$ in Random Mixing with Bleurt and BALD threshold $\tau_{BALD}$ in uncertainty-aware selection (BALD) with Bleurt. We observe that with increase in both the hyperparameters, the query complexity decreases, \textit{i.e.}, with a greater amount of feedback received from Bleurt, the number of required human annotations is lower. However, as shown in figure \ref{fig:bleurt_vs_bleu}, the opposite trend holds when the evaluation metric is inaccurate such as Bleu in MT tasks. In such cases, we are required to obtain a greater number of human annotations to compensate for the erroneous feedback received from the evaluation metric.

% \subsection{Robustness to Delayed Feedback}
% In some instances, human annotations are obtained from multiple crowdsourced annotators in parallel to reduce the time taken for annotations. In such cases, the online learner $\Gamma$ is required to choose the system pairs $(a_{t}^{(1)}, a_{t}^{(2)})$ to give to some annotator $i$ even before we obtain the result ${w}_{t-1}$ of the previous comparison from some other annotator $j$. In other words, the online learner may experience a delay $d > 0$ in feedback where at time $t$, the learner may only have access to the comparison history $\mathcal{H}_{t-d-1}$. As shown in figure \ref{fig:feedback_delay}, we observe that the top-performing dueling bandit algorithms tend to be robust to delays in feedback. We notice that the variation in query complexity of RMED and RCS as measured by standard deviation is just 64.49 and 62.86, respectively.

% Interestingly, we observe that RCS, RUCB, DTS, and DTS++ are more robust to feedback delays than RMED because they are stochastic algorithms and hence are able to alleviate the influence of delayed feedback by randomizing over actions. On the other hand, RMED is deterministic and is more affected by delays in feedback. % Given, these results we feel that the overall best strategy would be to use RMED when there is no delay in the feedback and to adopt the RCS algorithm  which performs very similar to RMED if delays in feedback are inevitable. 
% \MK{This was nice. One Q though. Does this cast doubts over our choice of using RMED. I mean will some reviewer pick this up and say ``Hey, looks like RMED is very sensitive then why did you use it in your experiments?'' SHould we end with a sentence that `we expect in most cases the annotator feedback can be synchronised and hence this is not a concern'' or ``Given, these results we feel that the overall best strategy would be to used RMED and ensure that there is no delay in the feedback''. Some sentence is needed at the end of this para.}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/wmt-16-deu-eng-delays.png}
%     \caption{Query Complexity vs delays in feedback on the WMT16 deu-eng dataset}
%     \label{fig:feedback_delay}
% \end{figure}


==> tables/task_and_datasets_assumptions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|l|c|c|c|c|c|c|c|c}
\Xhline{3\arrayrulewidth}
\multicolumn{1}{c|}{}                                                                   & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                             & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{}                                                                                         & \multicolumn{5}{c}{Assumptions}                                                                                                                                                       \\ \cline{6-10} 
\multicolumn{1}{c|}{\multirow{-2}{*}{Task}}                                             & \multicolumn{1}{c|}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\# Systems}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\# Human \\ Annotations\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Label Distribution\\(0-0.5-1)\end{tabular}}} & \multicolumn{1}{c|}{TO} & \multicolumn{1}{c|}{CW} & \multicolumn{1}{c|}{SST}     & \multicolumn{1}{c|}{RST}     & \multicolumn{1}{c}{STI}     \\ \hline
                                                                                           & WMT15 fin$\rightarrow$eng                                  & 14                                                & 31577                                                                                                  & 37\%-26\%-37\%                                                                                             & True                                                  & True                    & {\color[HTML]{C00000} False} & True                         & {\color[HTML]{C00000} False} \\
                                                                                           & WMT15 rus$\rightarrow$eng                                  & 13                                                & 44539                                                                                                  & 36\%-27\%-37\%                                                                                             & {\color[HTML]{C00000} False}   & True                    & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} \\
                                                                                           & WMT15 deu$\rightarrow$eng                                  & 13                                                & 40535                                                                                                  & 32\%-36\%-32\%                                                                                             & {\color[HTML]{C00000} False}                          & True                    & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} \\
                                                                                           & WMT16 tur$\rightarrow$eng                                  & 9                                                 & 10188                                                                                                  & 28\%-44\%-28\%                                                                                             & True                                                  & True                    & {\color[HTML]{C00000} False} & True                         & {\color[HTML]{C00000} False} \\
                                                                                           & WMT16 ron$\rightarrow$eng                                  & 7                                                 & 15822                                                                                                  & 38\%-24\%-38\%                                                                                             & True                                                  & True                    & True                         & True                         & {\color[HTML]{C00000} False} \\
                                                                                           & WMT16 cze$\rightarrow$eng                                  & 12                                                & 125788                                                                                                 & 38\%-25\%-37\%                                                                                             & True                                                  & True                    & {\color[HTML]{C00000} False} & True                         & {\color[HTML]{C00000} False} \\
\multirow{-7}{*}{\begin{tabular}[c]{@{}l@{}}Machine\\ Translation\end{tabular}}            & WMT16 deu$\rightarrow$eng                                  & 10                                                & 20937                                                                                                  & 37\%-26\%-37\%                                                                                             & {\color[HTML]{C00000} False}                          & True                    & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} \\ \hline
                                                                                           & Grammarly (FCE)                                & 7                                                 & 968                                                                                                    & 29\%-40\%-31\%                                                                                             & True                                                    & True                    & {\color[HTML]{C00000} False} & True                         & {\color[HTML]{C00000} False} \\
                                                                                           & Grammarly (Wiki)                               & 7                                                 & 992                                                                                                    & 29\%-40\%-31\%                                                                                             & {\color[HTML]{C00000} False}                        & True                    & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} \\
\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Grammatical\\ Error\\ Correction\end{tabular}} & CoNLL-2014 Shared Task                         & 13                                                & 16209                                                                                                  & 23\%-52\%-25\%                                                                                             & {\color[HTML]{C00000} False}                        & True                    & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} \\ \hline
Data-to-Text                        & E2E NLG Challenge                              & 16                                                & 2979                                                                                                   & 24\%-50\%-26\%                                                                                             & {\color[HTML]{C00000} False}    & True                    & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} \\ \hline
Paraphrase                            & ParaBank                                       & 28                                                & 151148                                                                                                 & 44\%-2\%-54\%                                                                                             & {\color[HTML]{C00000} False}   & True                    & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} \\ \hline
Summarization                     & TLDR OpenAI                                    & 11                                                & 4810                                                                                                   & 49\%-0\%-51\%                                                                                             & {\color[HTML]{C00000} False}                    & True                    & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} & {\color[HTML]{C00000} False} \\ \Xhline{3\arrayrulewidth}
\end{tabular}}
\caption{Dataset statistics along with the dueling bandit assumptions satisfied by the data}
\label{tab:dataset_stats_assumptions}
\end{table*}
